QUILT: Effective Multi-Class Classification on Quantum Computers Using an Ensemble of Diverse Quantum Classifiers

Quantum computers can theoretically have significant acceleration over classical computers; but, the near-future era of quantum computing is limited due to small number of qubits that are also error prone. Quilt is a framework for performing multi-class classification task designed to work effectively on current error-prone quantum computers. Quilt is evaluated with real quantum machines as well as with projected noise levels as quantum machines become more noise-free. Quilt demonstrates up to 85% multi-class classification accuracy with the MNIST dataset on a five-qubit system.

==> sections/background.tex <==
\section{Quantum Classification Background}

\textbf{Qubit and State Manipulation.} The qubit is the fundamental building block of a quantum computer. Where a classical bit is strictly binary, a qubit can be in a \textit{superposition} of both binary states, as shown below in Dirac notation:
\begin{equation}
\ket{\Psi} = \alpha\ket{0} + \beta\ket{1} \ s.t \ \ \alpha, \beta \in \mathbb{C} \ \& \ \ \norm{\alpha}^2 + \norm{\beta}^2 = 1
\end{equation}
Here, $\ket{\Psi}$ is the state of the qubit, which is in a superposition of the $\ket{0}$ and $\ket{1}$ basis states. When the qubit's state is measured, its superposition collapses and outputs state $\ket{0}$ with probability $\norm{\alpha}^2$ and $\ket{1}$ with probability $\norm{\beta}^2$.

Qubit states can be manipulated using unitary transformations that act as single- or multi-qubit quantum gates. Single-qubit gates are represented as rotation gates with three angle parameters: $R_3(\theta_1,\theta_2,\theta_3)$. Arbitrary superpositions can be achieved by tuning the rotation angles of this $R_3$ gate. Gates spanning multiple qubits have the ability to \textit{entangle} qubits into a unified quantum system.\vspace{2mm} 

\noindent\textbf{Quantum Circuits.} A quantum circuit is a sequence of gates applied to a system of qubits to affect the outcome of their entangled superposition state. \textit{All quantum gates in a quantum circuit can be represented using a unitary matrix $U$ such that $U^\dagger U = I$, where $U^\dagger$ is the complex conjugate transpose of $U$~\cite{quantum_text}}. As a quantum computing system can only undergo unitary transformations, all quantum circuit operations are completely reversible. The goal of this paper is to perform classification. On quantum computing systems, a specific type of quantum circuits -- quantum variational circuits (QVCs) -- have been used for classification tasks in place of classical neural networks due to their more efficient structure using far fewer parameters and their theorized exponential scaling properties over classical algorithms\cite{chen2020variational,Lockwood_Si_2020}. Therefore, next we briefly introduce the basic functions of QVCs. \vspace{2mm} 

\begin{figure}[t]
    \vspace{-4mm}
    \centering
    \includegraphics[scale=.46]{./figures/onevoneboth.pdf}
    \vspace{1mm}
    \hrule
    \vspace{1mm}
    \caption{State-of-the-art multi-class quantum classifiers have (a) quadratic scaling for number of models and (b) quickly degrading accuracy as the number of classes increase.}
    \vspace{-8mm}
    \label{fig:onevone}
\end{figure}

\noindent\textbf{Quantum Variational Circuits.} \textit{QVCs are tunable quantum circuits that can be optimized for a specific purpose through training~\cite{Schuld_2019}.} QVCs are built using a mix of fixed gates (e.g., single-qubit gates with fixed rotation angles), which encode fixed classical data $x$ (e.g., input features used for a classification task) and tunable gates (e.g., single-qubit gates with parameterized rotation angles), which encode objective function information $\theta$ (e.g., maximize classification accuracy). A function $f$ is then created to map these parameters $(x,\theta)$ to a quantum system. This function can be any series of unitary operations that define the unique circuit architecture, applied to the initial $\ket{0}$ state.
\begin{equation}
f(x,\theta) = U(x,\theta)\ket{0}
\label{eq:2}
\end{equation}
The parameters of this function are tuned via a hybrid classical-quantum computing approach for objective optimization~\cite{qvc_paper,Havl_ek_2019}. QVCs are entirely differentiable and can therefore, be optimized through standard deep learning optimization algorithms such as the Adam Optimizer~\cite{kingma2014adam}.\vspace{2mm}

\noindent\textbf{QVCs for Classification.} A classifier is a function mapping a point in input space $X$ to an output in label space $Y$. A classifier task must find a function $f(x)$ s.t: $f(x) = Y$, where $X \in {\Bbb R}^\mathbb{N}$ and $Y \in \mathbb{Z}$. QVCs are a suitable choice for a binary classifier as they provide high accuracy with few parameters, can be optimized with the same procedures as a neural network, and are small enough to fit on quantum machines today. A major challenge however is how to scale these classifiers to multi-class classification. Most real-world classification work done today involves more than two classes, but existing quantum classifiers are focused on solving only binary classification tasks and do not place much emphasis on multi-class classification tasks ~\cite{Schuld_2017} and~\cite{nature}.



%\red{XXX- I shuffled around stuff and removed the classical part from here - now we need more stuff under this heading; more details about how a SINGLE QVC can be used to perform binary classification  add a sentence about the challenges in using QVC for classification. make it clear why QVC is the obvious choice for doing classification and then, point out the challenge. ---XXX.}

%chen2020variational
%In this paper, we demonstrate how a QVCs can be effectively 


%As we demonstrate in this paper, QVCs can prove to be an efficient alternative. XXX-- 

%Before a QVC can be applied to an $n$-qubit quantum system, it is initialized to the ground state $\ket{0^{\otimes n}}$, which we simply represent as $\ket{0}$. Then, the state preparation circuit is applied to add the fixed classical data $x$ (input features vector of length $2^n$) to the circuit, such that each input feature is embedded into the amplitude of individual quantum states. The system state after this point can be represented as:
%\begin{equation}
%\ket{\psi} = \sum_{n=0}^{{2^n}-1}x_n\ket{n}
%\end{equation}

%A qubit is the building block of quantum computing. Where a bit is either in state 0 or 1 at any given time, a qubit can be viewed as a superposition of 0 and 1. The state for a single qubit is thus defined by:
%\begin{equation}
%\ket{\Psi} = \alpha\ket{0} + \beta\ket{1} s.t \abs{\alpha}^2 + \abs{\beta}^2 = 1
%\end{equation}
%For example, a valid superposition state which, when measured, will give the result 0 half of the time and 1, the other half of the time is:
%\begin{equation}
%\ket{\Psi} = \frac{1}{\sqrt{2}}\ket{0} + \frac{1}{\sqrt{2}}\ket{1}
%\end{equation}

%These qubits can be manipulated manipulated by unitary transformations, which act as quantum logic gates. This is the same as a classical logic gate acting on a classical bit.
%A unitary matrix is one that satisfies the constraint \cite{quantum_text}
%\begin{equation}
%U^\dagger U^{-1} = I
%\end{equation}
%Abiding by this unitary constraint also enforces full reversibility for the circuit.  This is a unique feature of quantum circuits. A qubit maintains its superposition until it has been measured, upon which it assumes one basis state or another.

%\subsubsection{Quantum Circuits}
%A quantum circuit is a series of gates being applied to a system of qubits to affect the outcome of their entangled superposition state. Quantum logic gates can act on any number of qubits.  For example a CNOT gate is a two-qubit gate that flips the second qubit only if the first qubit is a $\ket{1}$. Once a measurement operation is performed on the qubits, they will collapse each qubit to a state of $\ket{0}$ or $\ket{1}$ with a probability defined based on the operations in the circuit.  The state $\ket{\Psi}$ is measured according to the underlying probabilities of $\abs{\alpha^2}$ and $\abs{\beta^2}$.

%\subsubsection{Quantum Variational Circuits}
%Quantum Variational Circuits \cite{Schuld_2019} (QVC) are tunable quantum circuits, can be optimized through training. QVCs can use amplitude embedding to encode normalized input vectors on qubits.  The first step of state preperation to load classical data on quantum machiens is to reset all states to a ground state $\ket{0}$.  Then
%the state preparation circuit $U_{\psi}$ transforms the normalized input vectors $x$ of length $n$.


%\begin{equation}
%U_{\psi}: \ket{\psi} = \sum_{n=0}^{{2^n}-1}x_n\ket{n}
%\end{equation}




%QVCs are built using a mix of fixed gates which encode fixed classical data $x$, and parametrized gates which encode tunable classical data $\theta$. These are tuned by small rotations via hybrid classical-quantum computing \cite{qvc_paper}, \cite{Havl_ek_2019}. A function is then created to map the classical gate parameters $(x,\theta)$ to quantum space. This function can be any series of unitary operations that define the unique circuit architecture.

%\begin{equation}
%f(x,\theta) = U(x,\theta)\ket{0}
%\end{equation}

%These circuits are entirely differntiable,  meaning they can be optimized through standard deep learning optimisation algorithms such as Adam Optimizer \cite{kingma2014adam}.
%\subsection{Classification via Supervised Learning}
%A classifier can be viewed as a function mapping a point in input space X to an output in label space Y.  The objective function in a classification must find a function $f(x)$ s.t:
%$f(x) = Y$
%where $X \in {\Bbb R}^\mathbb{D}$ and $Y \in \mathbb{Z}$
%\newline
%In this case Y represents a label to represent a class in all set of classes in the model. Many statistical methods can be employed to solve these sorts of classifications such as the use of a Gaussian Mixture Model \cite{chatzis2008signal}; however deep learning is more suited for more complicated problem spaces.
%Deep learning accelerates the process of solving the problem of classification by providing a polynomial approximation using the power of neural networks. 


==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:concl}

In this paper, we proposed \sol{}, an ensemble-based end-to-end multi-class image classifier for NISQ machines. We showed the scalability potential of \sol{} compared to other methods and demonstrated a significant improvement over the state-of-the-art in terms of accuracy and resource requirements. We also showed that these models can be run on today's quantum machines and project the improvements of \sol{} as quantum machines become more error-resistant.


==> sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evalu}

\subsection{Experimental Methodology}

\noindent\textbf{Dataset.} We evaluate \sol{} with the MNIST \cite{mnist}, Fashion-MNIST \cite{xiao2017/online}, and Cifar \cite{cifar} datasets, using an 80/20 training-to-testing split. MNIST is a greyscale digit dataset that is widely used for quantum classification \cite{nature,wilson2018quantum,PhysRevA.101.062327,Li_Song_Wang_2021,Tiwari_Melucci_2019}. We also use Fashion-MNIST and Cifar due to the greater difficult of classifying them than MNIST. For example, Cifar has more pixels than MNIST and is also in RGB. We use classes [\{(0, 1), 6, 7\}, 2, 3, 4, 5] for MNIST, [\{(t-shirt/top, trouser), pullover, dress\}, coat, sandal, shirt, sneaker] for Fashion-MNIST, and [\{(airplane, automobile), bird, cat\}, deer, dog, frog, horse] for Cifar. Here, the class sets used for two-class, four-class, and eight-class classification are enclosed in (), \{\}, and [], respectively. We refer to these classes using the naming convention ``$<$dataset$>$-$<$classes$>$'' (e.g., Cifar-8 for eight-class Cifar).\vspace{1mm}

%We evaluate \sol{} with the MNIST \cite{mnist}, Fashion-MNIST \cite{xiao2017/online}, and Cifar \cite{cifar} datasets. We chose these datasets as they are widely used to establish baselines.  MNIST is the most commonly used and has been used in quantum classification work in the past \cite{nature,wilson2018quantum,PhysRevA.101.062327}, while Fashion-MNIST and Cifar are less commonly used. We chose to test for Cifar as well to give an added level of difficulty to the classification.  Cifar has more pixels than MNIST and Fashion-MNIST, but also has an RGB color-scale which presents more information than a gray-scale image.  As all of our datasets are reduced to 32 features, inevitably more data is lost for the Cifar dataset, which makes the classification harder. For binary classification, we use 0's and 1's from the MNIST dataset, T-shirts and Trousers from Fashion-MNIST, and Airplanes and Automobiles from Cifar. For 4 classes, we use MNIST classes [0, 8, 7, 1], Fashion-MNIST classes [T-shirt/top, Trouser, Pullover, Dress] and Cifar classes [airplane, automobile, bird, cat].  For 8-class classification we use [0, 1, 2, 3, 4, 5, 6, 7] for MNIST, 	[T-shirt/top, Trouser, Pullover, Dress, Coat, Sandal, Shirt, Sneaker] for Fashion-MNIST, and [airplane, automobile, bird, cat, deer, dog, frog, horse] for Cifar. We refer to these classes using the naming convention dataset-classes (e.g., Cifar-8 for 8-class Cifar classification).\vspace{2mm}

\noindent\textbf{Setup Details.} Our solution environment uses Python3, with Pennylane \cite{pennylane} as a framework using Qiskit \cite{Qiskit} as the backbone. We use Sklearn to perform PCA preprocessing for our datasets. Our noise-free simulations take place using the default Pennylane backened simulator. For our noisy simulations, we use ``qiskit.aer'' to set the error rates of quantum gates. Our real machine evaluations are run on IBM's five-qubit Lima and Manila computers.\vspace{1mm}

\noindent\textbf{Comparative Techniques.} (1) \textbf{OneVsOne:} As introduced in Fig.~\ref{fig:onevone}, this current state-of-the-art technique performs multi-class classification by combining many binary classifiers for a multi-class decision. This is the extension of ~\cite{nature}. (2) \textbf{Ensemble:} The ensemble is similar to \sol{}, but without the OneVsAll classifiers or multiple variants. Each member is responsible for a bit of the classification, allowing the binary classifier to scale to multi-class. There are five of these members for each bit and the decision procedure is a simple majority rules. \textit{We include this method for a comparison to show why off-the-shelf ensemble methods are not sufficient for multi-class classification.} We use the same PCA-based dataset preprocessing technique as \sol{} for the competitive techniques for fair comparison. %Quantum image classification is a less explored field are requires different solutions from the classical world.
% This ensemble approach is an earlier iteration of \sol{}.%The ensemble technique is the simplest classical to quantum conversion of an ensemble. The ensemble is constructed of binary QVCs mentioned in previous works. Each of these members is responsible for a bit of the classification, allowing the binary classifier to scale to multiclass.  There are 5 of these members for each bit and the decision procedure is a simple majority rules.  This ensemble approach is an earlier iteration of \sol{}.

\subsection{Results and Analysis}

\begin{figure}[t]
    \centering
    \includegraphics[scale=.52]{./figures/mnist_all.pdf}
    \vspace{0mm}
    \hrule
    \vspace{1mm}
    \caption{\sol{} scales better to higher number of classes than comparative techniques for the MNIST dataset.}
    \vspace{-8mm}
    \label{mnistall}
\end{figure}

\noindent\textbf{\sol{} achieves higher accuracy than comparative state-of-the-art techniques as the number of classes increases.} We show classification accuracy for MNIST-2, MNIST-4, and MNIST-8 in Fig. \ref{mnistall}. We make several observations. We note that all methods perform similarly on 2 classes as binary classification is a relatively simpler task. However, \sol{} provides 22\% and 46\% point better classification accuracy over the state-of-the-art OneVsOne method as the number of classes increases to four and eight. This is because the accuracy-weighted ensemble allows \sol{} to factor in model accuracy, allowing more accurate models to be favored. Additionally, \sol{} consolidates classification to an ensemble, where each model is responsible for classifying all classes on its own, therefore making better use of the full capacity of the QVC: \textit{where \sol{} only requires 13 circuits for eight-class classification, the state-of-the-art OneVsOne classifier requires 28}. However, having an ensemble is not enough; by checking the error-prone bits, \sol{} is able to effectively treat one of the bits in each bad sample and obtain higher accuracy than the ensemble method. Even though the simple ensemble approach requires fewer models (i.e., $5$), we find \sol{}'s linear increase in the number of models with the number of classes to be justified given the significant increase in accuracy.\vspace{1mm}


%While a one-bit error check is enough for eight classes with three qubits, it will likely be necessary to error check more bits as more qubits are introduced to the circuit.

\begin{figure}[t]
    \centering
    \includegraphics[scale=.52]{./figures/4classes.pdf}
    \vspace{0mm}
    \hrule
    \vspace{1mm}
    \caption{\sol{}'s accuracy is considerably better than other methods for all well-known (a) four-class and (b) eight-class datasets.}
    \vspace{-7mm}
    \label{4digit}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[scale=.49]{./figures/differentarc.pdf}
    \vspace{0mm}
    \hrule
    \vspace{1mm}
    \caption{An ensemble with multiple different variants performs better than one with multiple instances of one variant (MNIST-4). The figure shows the results when using just the ensemble to remove the impact of the OneVsAll error-correcting classifiers.}
    \vspace{-8mm}
    \label{samevsdifferentarc}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[scale=.52]{./figures/4classesreal.pdf}
    \vspace{0mm}
    \hrule
    \vspace{1mm}
    \caption{(a) MNIST-4 and (b) MNIST-8 accuracy on IBM's quantum machines Lima and Manila along with a simulated interpolation based on half of Manila's noise levels. OneVsOne could not be computed for eight classes on the real machines as it required an impractical number of model evaluations.}
    \vspace{-7mm}
    \label{real-4}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[scale=.49]{./figures/simulated_acc.pdf}
    \vspace{0mm}
    \hrule
    \vspace{1mm}
    \caption{Projected increase in MNIST-8 accuracy as the hardware noise decreases with evolution in quantum computing technology.}
    \vspace{-8mm}
    \label{simulatednoise}
\end{figure}

\noindent\textbf{\sol{} outperforms competitive techniques across multiple well-known deep learning image datasets.} In  Fig. \ref{4digit}(a), we evaluate how well \sol{} performs on Fashion-MNIST-4 and Cifar-4, in addition to MNIST-4.  We also look at how \sol{} compares to other solutions. \sol{} outperforms the state-of-the-art by 46\%, 38\%, and 14\% for MNIST-8, Fashion-MNIST-8, and Cifar-8, respectively. All methods perform better on Fashion-MNIST-4 and MNIST-4 than on Cifar-4. This is because of the limited size of the encoded data that makes encoding the RGB images in Cifar-4 into 32 features tougher (i.e., more information is lost by performing PCA on Cifar images). We also evaluate performance of different datasets for eight classes in Fig. \ref{4digit}(b) and observe similar behavior. Comparing the two figures demonstrates that \sol{} is the most scalable and highest performing solution across different datasets.\vspace{1mm}

\noindent\textbf{\sol{}'s strategy of using multiple variants achieves significantly higher accuracy than using a single variant.} Fig. \ref{samevsdifferentarc} confirms \sol{}'s critical design component: higher accuracy is achieved by adding diversity to variant architectures in ensembles. While different instances of a homogeneous variant can be diversified using different initial weights, because these instances traverse the same hyper-dimensional space during parameter optimization, they cannot provide the level of diversity of heterogeneous variants.\vspace{2mm}

%The weights are trained classically, then uploaded to be run using real IBM quantum machines.  -- this is a methodology detail. If it needs to be included, it needs to go there. 

\noindent\textbf{\sol{} outperforms other techniques on running image classification tasks on today's noisy real quantum machines.} Fig. \ref{real-4} (a) and (b) show \sol{}'s classification accuracy for MNIST-4 and MNIST-8 datasets on real quantum computers. \sol{} outperforms other methods due to the redundancies built into it that were designed to make it work well on small and noisy circuits. While we do not focus our optimizations on the noisy machines of today, we still abide by the constraints that allow \sol{} to be executable on today's quantum machines. We also note that the overall accuracy on real systems in lower than our previous simulated results due to the hardware noise. However, in the future, the noise is expected to reduce significantly, with estimates such as $10^{-4}$ error rate ~\cite{Jurcevic_2021}. \vspace{2mm}

\noindent\textbf{\sol{}'s accuracy performance will only improve with reduction in hardware noise levels as quantum technology advances.} We simulate several noise levels between the ideal case of 0 and the current case of real machines and show how different levels of noise affect the accuracy. Fig. \ref{simulatednoise} demonstrates that as noise levels continue to improve on real NISQ devices, the accuracy of \sol{} improves. It should be noted that the accuracy on real machines can be improved significantly by reducing the size of the network. However, this significantly impacts the accuracy in simulation and on future low-noise machines.

%As we wish \sol{} to be applicable and usable as NISQ technology progresses, we did not specifically optimize \sol{} for today's real machines. Instead, we primarily focused our efforts on scalable quantum simulations and multi-class classification performance.



==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

\textbf{Problem Motivation.} Quantum algorithms have been developed in the areas of chemistry, cryptography, machine learning, and optimization~\cite{Lu_Liu_Wang_Huang_Lin_He_2019,shor,Tiwari_Melucci_2019,Khairy_Shaydulin_Cincio_Alexeev_Balaprakash_2020}. A class of algorithms known as quantum variational algorithms are designed to optimize and execute quantum machine learning and classification workloads~\cite{qvc_paper}. 

While theoretically-promising, existing quantum machine learning classifiers are designed for future large-scale ideal quantum systems. This is because loading data, training, and testing samples on existing near-term intermediate-scale quantum (NISQ) computers is challenging due to significant hardware errors~\cite{schuld2019quantum,Jurcevic_2021,Preskill2018quantumcomputingin}. \emph{Consequently, existing quantum classifiers have been demonstrated to be effective only for relatively simple binary classification tasks~\cite{Schuld_2017,nature}. As our evaluation confirms, existing state-of-the-art approach are ineffective for multi-class classification (e.g., $<$30\% accuracy for eight-class image classification). Currently, there is lack of capability to perform multi-class classification tasks on the real quantum machines for exploration and improvement.}\vspace{2mm}

\noindent\textbf{Contributions.} \sol{} specifically bridges this gap by open-sourcing its framework and dataset to the community for multi-class classification on NISQ quantum machines. \sol{} makes the following key contributions:\vspace{2mm} 

(1) A key idea behind \sol{} is to build an ensemble of quantum classifiers to perform multi-class classification. While intuitive and widely-applied in the classical world, we found that classical way of building ensembles is ineffective -- it improves the accuracy only by 5\%-10\% over the state of the art. To mitigate this challenge, \sol{} builds a novel ensemble of quantum classifiers by (1) constructing diverse classifiers, and (2) keeping them simple.

(2) Second, we demonstrate that \sol{} further enhances the classification accuracy obtained via carefully constructed diverse ensembles of models. \sol{} makes an observation that when outputs from diverse models are combined, individual models agree on ``most parts'' of the output, but they may disagree on ``some parts'' due to the intrinsic noise, which cannot be mitigated simply by increasing the diversity or number of members. To mitigate this, \sol{} designs a safeguard error correcting mechanism that detects which parts have most disagreement and then, builds specific error-correcting binary classifiers to increase the consensus for those parts, improving the overall prediction accuracy. 

(3) Third, we show how \sol{} performs on a variety of datasets and in different simulation environments. We evaluate \sol{} on MNIST, Fashion-MNIST, and Cifar for four and 8 classes. \sol{} demonstrates an advantage in every case by up to 46\% over state-of-the-art for eight classes of MNIST.  We also demonstrate that \sol{} can be run on real quantum machines today and test on IBM Manila and IBM Lima. We also examine how accuracy scales for \sol{} for different levels of noise.

%XXX--In particular, include key quantitative results state IBM machine names too, state as improvement percent point over state of the art, for high number of classes, mention data set names--XXX.


%\sol{} uses a hybrid classical-quantum approach to mitigate the data loading challenge and erroneous nature of quantum machines. The training is partially done on the quantum simulator for faster training to mitigate the challenge of loading large data, but the training is also augmented by doing a part of the training on the error-prone, real quantum machines to account the effects of errors to improve the classification accuracy of the inference tasks on real quantum machines.\newline 

%(2) To mitigate the effects of errors, \sol{} performs the partial training and testing (inference) tasks on a pool of quantum machines instead of a single machine. While the idea of building a pool of classifiers has been applied in the classical machine learning tasks, we found that applying this idea as-is in the quantum machine learning context does not provide any benefit without mitigating quantum-specific challenges which have no classical analogy. For example, to make the pool effective, OPTIC builds an optimizer to disperse the observed Pauli-Z measurements for different quantum machines as real machines do not display the ideal dispersion characteristics of the designed model.\newline 



==> sections/misc.tex <==
\subsection{Miscellaneous Work}
\subsubsection{One Vs One Classifier}
A frequently mentioned and perhaps intuitive extension from binary classification to multi-class is to use the One Vs One Classifier.  This method allows multi-class classification by creating many binary classifiers, then combining them all for a multiclass decision. In the case of a 3 class classification with classes A, B, and C, this would require 3 unique classifiers; for (A,B), (B,C), and (A,C).
The number of classifiers required to build an n class multiclass classifier is 
\newline
$N=n(n-1)/2$

\subsubsection{Partial Binary Classifiers}
While One vs One classifiers fulfill this multiclass classification constraint of only working with reliable binary classifiers, scalability problems make this technique impractical. These issues can be seen in Figure \ref{onevone}

\begin{figure}[t]
    \centering
    \includegraphics[scale=.3]{./figures/onevone.png}
    \vspace{1mm}
    \hrule
    \vspace{1mm}
    \caption{}
    \vspace{-5mm}
    \label{onevone}
\end{figure}

\subsubsection{$L_0$ Loss}
It is also worth mentioning our work in trying to incorporate a sparsity based loss function. The idea behind this being to reduce the number of tunable parameters in an effort to reduce noise through a more robust network. We base this on the work in \cite{l0}, where pruning a neural network to set certain low-impact weights to 0, then re-training, creates a more robust network that is less susceptible to noise.  The intuition being that certain weights do most of the learning, with the underlying solution being sparse, and by slowly removing the unnecessary weights, a smaller network can exist with less noise.  We found that attempting to enforce sparsity in these already small networks disturbed the network to much, leading us to believe that due to the small size of these networks, every weights is very important.  Even a slight perturbation in weights through pruning essentially reset the entire training of the network and for this reason we do not recommend enforcing sparsity in NISQ networks.  Perhaps when networks are allowed to get much larger and there exists room for this noise, an L0 norm would be useful to incorporate.
\subsection{Results from Bitwise Classifiers}
It is also worth mentioning our work in splitting each standard classifier into individual bitwise classifiers.  Overall, these tended to have a lower accuracy, but are useful as they enable scaling to even more classes.  In this case, each bitwise classifier performs a subgroup classification, splitting the data in half. 
We test this with different variations of bitwise classifiers.  We first test using only a single classifier for each bit to establish a control for our other improvements.  We then use an ensemble of size 3 and a standard majority rules decision procedure in order to increase the accuracy.  We also show results for the more advanced decision procedures of using a best 2 out of 3 for the bitwise classifiers, inclusive classifiers, and exclusive classifiers.  Finally we show the accuracy for the more advanced hierarchical decision procedure based on the confidence levels we outline above.This can be seen in Figure 




\subsubsection{Ensemble Methods for Classification}
One common method for leveraging smaller circuits to create a better model is called an ensemble. Many methods have been proposed for using ensemble classifiers in quantum networks \cite{ensemble1},\cite{ensemble2}.  In general, an ensemble network uses a "panel of judges" approach where many judges evaluate the input though their own classifier and together come up with a solution that is better than what a single judge could accomplish.  This is based on the rather old The Cordocet Jury Theorem, originating in the year 1758.  This theorem states that if each judge has a probability of guessing correctly of over .5, then as the number of judges approaches infinity, the combined correct guess probability will approach 1.
There is much research on classical ensembles and while there are perhaps more optimal weighting procedures, we opt to use accuracy as a weighting mechanism, as opposed to the standard majority rules. The general formula for the ensemble output $\hat{y}$ based on the ensemble of judges for each judge ${\epsilon}$ in a majority rules decision rule is:
\begin{equation}
\hat{y} = sgn(\sum_{\epsilon} f(\hat{x}, \theta))
\end{equation}

This panel guess can be thought of as the weighted sum of each classifier $f(\hat{x}, \theta)$ where the $sgn$ is the sign function that will convert anything less that 0 to 0, signifying a guess of class 0, and anything greater than 0 to 1, representing class 1 as the guess.  In the case where a weight mechanism is used,each judge has an associated weights,and thus $w_\theta$ will be added to the ensemble function equation.  This equation is shown below:

\begin{equation}
\hat{y} = sgn(\sum_{\epsilon} w_\theta f(\hat{x}, \theta))
\end{equation}


 
\subsection{Quantum Data Encoding Problem}
An open question in quantum computing is how to efficiently load in classical data into quantum machines \cite{fine_print}.  The range of proposed solutions are outside the scope of this paper, however it should be noted this is a tough problem that must be faced in quantum algorithms. For example, even in using the relatively small MNIST images, 784 bits of information must be encoded on a quantum machine, which only contain at most 10s of qubits.  This poses a serious problem in 3 ways.  First, even if 784 qubit machines existed today, it would be an arduous task to use any method, including amplitude embedding, to encode all of this information accurately on a quantum machine. Secondly, as the amount of qubits introduced to a system increases, so does the total amount of noise in the system, which impacts the learning and inference procedure of the supervised learning attempt.  Lastly, and perhaps most obviously, no 784 qubit computers exist as of today, so encoding an entire MNIST image in a quantum computer in one read, would be impossible.

==> sections/motivation.tex <==
\section{Motivation for \sol{}}
\label{sec:motiv}

Quantum computing can have exponential acceleration over classical computers in many problem domains~\cite{shor,3body,many-body, qml,PhysRevLett.83.5162,Lu_Liu_Wang_Huang_Lin_He_2019}. Notably, quantum computing is also expected to prove useful for the field of machine learning and classification \cite{qml, fine_print,Lockwood_Si_2020, chen2020variational,Yang_Jiang_Zhang_Sun_2020,Li_Gkoumas_Sordoni_Nie_Melucci_2021,Khairy_Shaydulin_Cincio_Alexeev_Balaprakash_2020}. While new discoveries have led to better quantum machines, a defining limitation of the near-term noisy intermediate-scale quantum (NISQ) computers is the lack of large fault-tolerant  machines. One is therefore limited to using only a handful of qubits to perform quantum algorithms. This largely constrains the development of quantum algorithms for real-world applications. \textit{In this section, we outline some of the challenges in the current state of research in NISQ computing that pertain to classification problems, and how \sol{} is designed to effectively utilize existing small-scale NISQ hardware to perform classification tasks accurately.}

\begin{figure*}
\centering
  \includegraphics[scale=0.18]{./figures/flow.pdf}
     \vspace{1mm}
  \hrule
\vspace{1mm}
  \caption{Overview of the design of \sol{}. The label under each step indicates whether the step is performed quantumly or classically.}
  \label{flow}
    \vspace{-8mm}
\end{figure*}

\subsection{Related Quantum Classification Efforts}

Multiple works have been put forward in the space of quantum image classification. For example, \cite{gambs2008quantum}, \cite{PhysRevLett.118.190503}, and \cite{wang2021quantum} are focused on theoretical algorithms that can only run on large fault-tolerant quantum computers; while promising, these works are not applicable in the current NISQ era as the computers are small and noisy. Other works leverage classical neural networks to handle much of the heavy lifting for quantum classification~\cite{8638596,9425825}. Unfortunately, in these cases, the potential for quantum speedup is greatly reduced as the works inherit the limitations of classical networks, such as when dealing with data in quantum entangled states \cite{nature}.

The most relevant and recent efforts in the quantum classification space are~\cite{Schuld_2017} and~\cite{nature}. These efforts are state-of-the-art effort for classification tasks on NISQ quantum computers. In \cite{Schuld_2017}, the authors use a simple distance-based classifier in simulation to classify the Iris dataset by analyzing how it performs for each pair of classes (1v2, 2v3, and 1v3) in separate binary classifications. The more recent work -- \cite{nature} -- tackles the same image classification problem of splitting the Iris dataset into tuples, with the addition of analyzing binary splits in the MNIST dataset. They use tensor networks to build their binary classifiers, then evaluate the performance on a real quantum computer. However, both~\cite{Schuld_2017} and~\cite{nature} are primarily designed to be effective for binary classification. While they attempt to extend to multi-class classification using binary classifications on every unique two-class pairing in their datasets, this ad-hoc extension approach has several limitations, as we discuss next and our evaluation confirms. 



\subsection{Why are the State-of-the-Art Quantum Classifiers Not Effective for Multi-Class Classification?}

The state-of-the-art approach for multi-class classification~\cite{nature} essentially relies on splitting a multi-class dataset into many binary datasets and classifying each pair and combining them all for a multi-class decision -- known as the OneVsOne Classifier. For example, for a three-class classification with classes A, B, and C, this would require three unique classifiers; for (A,B), (B,C), and (A,C). Each one votes in favor of one class and the class with two votes wins. However, this method has several shortcomings.

First, \textit{the current approach suffers from poor scalability as a large number of models are needed for training.} The number of models required to build an $n$-class multi-class classifier is $n(n-1)/2$ (Fig.~\ref{fig:onevone}(a)). Each model that needs to be trained classically slows down training significantly. Additionally, the inference on quantum machines becomes impractical with larger number of classes. For example, 8 classes would require 28 models, and 16 classes would require 120 different models to be initialized on quantum computers. Instead, \textit{\sol{}, as we discuss later, is designed to scale only linearly with the number of classes}. % 

Second, \textit{the accuracy of the current approach degrades quickly with increase in the number of classes (Fig.~\ref{fig:onevone}(b)).} One reason for this is the well-documented issue for the OneVsOne classifier: the ``the unclassable region'' problem~\cite{galar2011overview, liu2007nesting}. This is where no obvious winner can be selected from the binary classification pairs; for example, a three-class scenario where two candidates tie with one vote each. As more classes are added, the opportunities for ties increase as well. In fact, each additional classifier brings more noise to the system and adds more points of failures if the classifier is biased to a particular class. For this reason, \textit{we design \sol{} with an ensemble of classifiers, where each classifier is wholly responsible to classify all classes}. 



%---- scratch space -----

%Overall, state-of-the-art quantum classification approach scale poorly with the number of classes. To this end, we are motivated to push multi-class quantum image classification to the next level in terms of scalability and accuracy. 

%The implications of an exponentially faster classification device would redefine the landscape of deep learning.

==> sections/related_work.tex <==
\section{Related Work}
Curated algorithms for classifying images on quantum machines is not a novel idea.  In fact, there have been a few attempts in the last few years such as \cite{mnist} and \cite{rnn}. \cite{mnist} proposed a method that in simulations achieved a whopping 98.5\% accuracy. While this method maintains our approach of performing dimensionality reduction on the input MNIST images, it varies for some key reasons. Firstly this is not designed for nor has been run on real quantum machines.  6 TB of RAM was required to run this simulation and is impractical to run on today's NISQ machines, where as our experiments have been shown to run on relatively smaller quantum machines.  Additionally, we use Principal Component Analysis instead of the proposed dimensionality reduction technique of QSFA as it is a simpler algorithm and fits our purposes better. PCA is used to enable efficient compression that can be specified to any arbitrary size. This allows QUILT to fit on today’s NISQ machines and is mathematically the efficient way to encode data to maximize explained variance across a dataset. It is worth noting that other works such as \cite{henderson2020quanvolutional} have used threshold based encoding where pixel values above a certain threshold are encoded as the state $\ket{0}$ and those above are in the state  $\ket{1}$. While it is possible this may perform better for certain datasets such as MNIST where shade is not as important, this is not especially useful for more complex datasets.
Additionally,\cite{rnn} introduces a quantum-compatible recurrent neural network; however, this network is entirely simulated on a classical computer and thus has not been shown to be compatible on today's NISQ computers.  This method also only computes one pixel at a time and only performs binary classification, while our method is scalable to all classes in the MNIST dataset and only requires on pass of data for each judge in the ensemble. In \cite{9323065}, the authors were able to successfully use multiclass image classification using quantum ensembles and were the first to do so.  We improve on this idea by designing our architecture around an ensemble, with specific auxillary classifiers such as the inclusive and exclusive classifier along with heterogeneous architecture to ensure diversity between ensemble members. We believe our method is more practical in scale as the number of networks needed in our method requires a linear scaling to the number of classes in the classification, while the previous state-of-the-art requires quadratic scaling. 
\label{sec:relat}



==> sections/solution.tex <==
\section{\sol{}: Design and Implementation}
\label{sec:solut}

\textbf{Overview of the approach.} Fig.~\ref{flow} illustrates the overview of \sol{}. A key idea behind \sol{} is to use an ensemble of smaller classifier models instead of using a single large classifier model. This design decision is made to ensure that the impact of quantum operation errors -- which are prevalent on quantum real machines -- is minimized. Multiple lightweight simple models (referred to as ``core classifiers'') make the training and inference process simpler and reduce the impact of errors. In fact, at present, training and inferring large complex models is not feasible due to technological constraints and that is a major roadblock that \sol{} curbs. 

A small-sized ensemble model is potentially less powerful than a complex, heavyweight model and may produce lower accuracy results. Therefore, to improve the classification accuracy, \sol{} builds an ensemble in a unique way. As shown in the second stage of Fig.~\ref{flow}, each classifier outputs its classification prediction (three bits for an 8-class classification problem) and these inference results are combined across all classifiers by weighting according to their accuracies. As an efficiency measure, the already calculated outputs, \hat{x}, are used to calculate the accuracy after each iteration. We started with a withheld validation set (10\% of the data), but we robustly verified that it did not improve accuracy significantly; so we removed this calculation to save time. As we discuss in detail later, simply replicating the models is not sufficient for improving the accuracy. \sol{} specifically designs them to be ``different by construction''. Each core classifier can have multiple instances and variants that help diversify the ensemble. Model, variant, and instance design details are discussed later in this section. 

During the development of \sol{}, we discovered that building a diverse ensemble is also not sufficient. As the fourth stage of Fig.~\ref{flow} illustrates, when predictions across all classifiers are combined, some bits in the final predicted (e.g., one bit out of three bits for an 8-class prediction task) output may have low-confidence. This is despite careful selection and construction of individual core classifiers. To address this, \sol{} designs unique binary classifiers to improve the prediction confidence of low-confidence bits. For example, in Fig.~\ref{flow}, ``1 vs All'' and ``5 vs All'' are used because the most significant bit has the lowest confidence and hence, the only output possibility is a `1' or a `5' depending upon the other predicted bits. Finally, \sol{} combines the results to predict the target class in a multi-class setting.

Next, before we discuss the model design details of \sol{}, we discuss the data processing procedure.




%\sol{}'s design is based on hybrid quantum-classical computation powered by q. As shown in Fig. \ref{flow}, the first stage in \sol{} is the training stage where all classifiers in \sol{}'s ensemble are trained using a quantum simulator. Then, these classifiers' weights, along with the model and images are dispatched to quantum machines to perform inference on the test set. Next, the results are aggregated on a classical computer to obtain the level of confidence for each guess.  Afterwords, the least confident samples are sent back to a quantum computer to be analyzed for a potential bit flip. After these low confidence samples return back, the selection procedure is applied.


\begin{figure*}
    \centering
    \includegraphics[scale=0.3]{./figures/Circuit Diagram.pdf}
        \vspace{1mm}
        \hrule
            \vspace{1mm}
    \caption{General structure of the different circuit architectures of \sol{}. On the right are examples of multiple variants for core classifiers. The architectures are different so as to enhance the capabilities of the ensemble. On the left is the structure of the OneVsAll circuits. As they are all binary classifiers and have no need for a distinct architecture, they only use a single measurement qubit and have the same structure.}
    \label{circuit_diagram}
    \vspace{-8mm}
\end{figure*}

\subsection{Preprocessing and Embedding Images and Labels}

Running a quantum classifier on a small NISQ quantum machine requires loading and encoding classical data on the quantum computer in a scalable manner. \sol{} has selected the model size to be five qubits because models spanning a larger number of qubits increase the surface area of error and hence, risk lowering the overall accuracy. 
% although they are potentially more powerful in theory due to additional size and complexity

%As a rule, $n$ qubits can represent a feature size of $N = 2^n$. As an example, the state space for two qubits is 
%$\ket{\Psi} = \alpha_{00}\ket{00} + \alpha_{01}\ket{01} + \alpha_{10}\ket{10} + \alpha_{11}\ket{11}$.

% \begin{figure}[t]
%     \centering
%     \subfloat[][]{\includegraphics[scale=.465]{./figures/explainedvar.pdf}}\hfill
%     \subfloat[][]{\includegraphics[scale=.255]{./figures/reconstruct.pdf}}
%     \vspace{1mm}
%     \hrule
%     \vspace{1mm}
%     \caption{(a) Amount of explained variance encoded through PCA. Adding more and more qubits has diminishing returns because explained variance approaches 100\%. (b) Example of an MNIST image, reduced from 784 to 32 features, then reconstructed. As $log_232=5$, this image can be encoded onto a five-qubit machine.} %  The data encoded in this image is the information the quantum machine receives for it to classify.  Note: even with only ~4\% of the data after compression (and reconstruction for sake of visualization), the image is still human-recognizable.
%     \vspace{-8mm}
%     \label{explained_var}
% \end{figure}

\textit{\sol{}'s solution to encoding each image on a quantum machine is to perform Principal Component Analysis (PCA) on the entire dataset as a preprocessing procedure prior to training the model.} PCA allows particular specification for the exact number of dimensions for data reduction. PCA has a one-time offline overhead of processing the image data and generating the 32 features ($<1$ minute overhead even with serial processing of 60,000 MNIST images). This allows QUILT to fit on today’s NISQ machines and is the most efficient way to encode data to maximize explained variance across a dataset. It is worth noting that other works such as \cite{henderson2020quanvolutional} have used threshold based encoding where pixel values above a certain threshold are encoded as the state $\ket{0}$ and those above are in the state  $\ket{1}$. While it is possible this may perform well for certain datasets such as MNIST where color and shade are not as important, this should not be expected to perform well for more complex datasets where color is important.

% \sol{} is built off of 32 dimensions so that all of the data could be encoded on a single 5 qubit quantum machine.

%A graph showing the amount of data preserved in the form of explained variance for various numbers of qubits is shown in Fig. \ref{explained_var}(a). An example of a reconstructed MNIST image after being reduced to 32 principal components from 784 features, is shown in Fig. \ref{explained_var}(b). Even with only ~4\% of the data after compression (and reconstruction for sake of visualization), the image is still human-recognizable.
%While techniques such as Quantum PCA \cite{QPCA} exist to reduce the number of dimensions, we found PCA to be a suitable solution within the hybrid model to calculate the principal components a single time offline.

%Once the images are preprocessed, \sol{} uses amplitude embedding to encode the normalized input vectors on to the qubits. The first step of state preparation to load classical data on quantum machines is to initialize all qubits to the ground state: $\ket{0^{\otimes n}}$, which we simply represent as $\ket{0}$.  Then, the state preparation circuit ($U_x$) is applied to add the fixed classical data $x$ (input features vector of length $2^n$) to the circuit, such that each input feature is embedded into the amplitudes of the individual quantum states. The system state after this point can be represented as:
%\begin{equation}
%U_x\ket{0} = \sum_{n=0}^{{2^n}-1}x_n\ket{n}
%\end{equation}
%Once the circuit is prepared to this state, it can then be appended with the models designed by \sol{}.\vspace{2mm}

Once the images are preprocessed, \sol{} uses amplitude embedding to encode the normalized input vectors on to the qubits. Amplitude embedding transforms $L$ vectors of normalized classical data of size $N$ and encodes the data as a quantum state of size $log_2({NL})$.  The training set size affects the pre-processing step, but not the characteristics of individual quantum classifiers The first step of preparing classical data for quantum computation is to initialize all qubits to the ground state: $\ket{0}$.  Then, the state preparation circuit ($U_x$) is applied to add the fixed classical data to the circuit, embedding one input feature per quantum state amplitude. Once the state is prepared, \sol{}'s classification model can then be applied. 
\sol{} also preprocesses the labels to ensure compatibility with the quantum space. This requires selecting a value of \{-1,1\} for each bit representing the label. With the preprocessing step complete, we delve into the model design details of \sol{}.


%Due to the reversible nature of quantum circuits, the classical data can be retrieved from quantum space by reversing the operations on the circuit after obtaining the measurement expectation $\hat{B}$

%\begin{equation}
%f(x,\theta) = \bra{0}U^\dagger(x,\theta)\hat{B}U(x,\theta)\ket{0}
%\end{equation}
%This enables a hybrid classical-quantum computing model which is core to the design of \sol{}.

%\noindent\textbf{Processing Labels.} 


% While quantum ensembles for classification have been developed previously \cite{ensemble1,ensemble2}, 

\subsection{\sol{}'s Model Ensembles}

%A limitation of NISQ circuits is the small number of qubits and tunable parameters available (due to the requirement to use as few operations as possible for noise minimization). 

% This gives \sol{} the ability to improve its performance without the need for a large model, which would suffer from high noise on a NISQ machine.

Large and complex models can be used as a building block for classification, but they increase the likelihood of errors on error-prone NISQ machines. \textit{To mitigate this challenge, \sol{} builds on a base of small-sized circuits because smaller circuit size reduces the adverse impact of errors. In addition, to compensate for the small circuit size, \sol{} builds an ensemble of such models that work together to collectively improve the classification performance.} \sol{} uses accuracy as a weighting mechanism to aggregate the classifications of individual ensemble components. Each ensemble $\epsilon$ with weight $w_\epsilon$ contributes to the output $\hat{y}$ according to the following equation:
\begin{equation}
\hat{y} = sgn\Big[\sum_{\epsilon} w_\epsilon O(x, \theta)\Big]
\end{equation}
where the $sgn(z)$ operation is defined as 
\[
  sgn(z) = \left.
  \begin{cases}
    -1, & \text{for } z < 0 \\
     1, & \text{for } z > 0 
  \end{cases}
  \right\}
\]
and the output $O(x, \theta)$ is a real number between -1 and 1, with its absolute value suggesting the confidence of being a member of the -1 or 1 class. The output is the result of applying the $U(x,\theta)$ operator to the $\ket{0}$ state and measuring it, where $U$ is the unitary transformation applied to input $x$ and parameters $\theta$ (from Eq.~\ref{eq:2}).

The ensemble representation for a QVC then becomes
\begin{equation}
\hat{y} = sgn\Big[\sum_{\epsilon}\dfrac{a_\epsilon}{a}  O(x, \theta)\Big]
\label{eq:5}
\end{equation}
where $a_\epsilon$ is the associated accuracy of ensemble member $\epsilon$ and $a$ is the sum of all ensemble accuracies.

Next, we discuss the design of \sol{}'s ensemble models.

% These different structures serve to diversify the gradient-descent based training procedure.

\subsection{Model Construction}

%Fig. \ref{definitions} visually illustrates the definition of key components of \sol{}: model, variant, and instance. XXX--consider summarizing that figure, at least connect what a cire classifier is? because that is the next thing discussed and has no connection to previous lines: this is a must-fix.--XXXX.\vspace{2mm}


%A model is an entire quantum circuit with a single objective. 
%A variant of a model is has the same objective function, but differs on the %circuit level by having different tunable parameters. Additionally, each %variant requires its own training and is uniquely optimized.
%While variants have unique architectures, an instance of a model is a full %implementation of a model, if multiple instances are of the same variant, the %only difference between them is the random initialization of weights when %training begins. We visualize these definitions in Figure \ref{definitions}.


\noindent\textbf{Core Classifier.} The building block of \sol{}'s ensemble is the core classifier, which is designed to be able to classify all classes on its own (as opposed an ensemble of OneVsOne classifiers used for state-of-the-art multi-class classification). It consists of an amplitude embedding circuit, followed by repeating rotation gates on each qubit, then CNOT gates to entangle all qubits together, followed by a measurement on all output qubits. 

In classical computing, traditional neural networks perform classification by assigning a single class to an output neuron to then use a function such as Softmax to find the most likely candidate. \textit{\sol{} uses a different approach by leveraging the quantum nature of the model: it uses each measurement qubit $b$ as a bit in the full $n$-bit classification. This allows better scaling to handle a larger number of classes.} All measurement qubits form a single bitstring that has an associated class label:
\begin{equation}
\hat{y} = \sum_{b=0}^{n}2^{n-b}\Big(\dfrac{sgn(q_b)+1}{2}\Big)
\end{equation}
Here, $q_b$ is the value of the $b^{th}$ bit as measured in the quantum state output (Eq.~\ref{eq:5}). The number of these models scale logarithmically with the number of classes in the label space $n=log_2{N}$, but the accuracy scales inversely. This is partially because in order for the entire output to be correct, all the bits have to be correct. For example, if each bit is correct with probability .95, the probability of a correct guess for a three-bit classifier would be $.95^3 = .857$ or 85.7\%.\vspace{2mm} 

\begin{figure}[t]
\centering
  \includegraphics[scale=0.17]{./figures/Definitions.pdf}
      \vspace{1mm}
  \hrule
      \vspace{1mm}
  \caption{Ensemble diversity hierarchy. At the top of the hierarchy is the \textbf{model}, which represents a quantum circuit with a unique objective. An example of this would be a OneVsOne classifier with the objective of distinguishing Trousers and T-Shirts. A model can have multiple \textbf{variants}, which are circuits with the same objective, but different structures. Finally, a variant can have multiple \textbf{instances}. All instances associated with a variant have the same structure, but may differ in their parameters due to different initial conditions used for optimization.}
  \label{definitions}
    \vspace{-8mm}
\end{figure}

\noindent\textbf{Multiple Diverse Variants of Core Classifiers.} Now that we have the general structure for a core classifier defined, our next task is to use this general structure to form an ensemble. It is imperative to diversify the ensemble components as much as possible in order to ensure that they correct for each other's deficiencies, blind spots, and biases. Initializing model instances with different initial conditions enforces some degree of diversity. However, these instances would still be optimizing over the same search space due to the model structure being the same, thus resulting in similar outputs and reduced ensemble diversity.

\sol{} mitigates this challenge by constructing model variants with heterogeneous architectures in order to establish more diversity and independence between them. These variants differ in that each variant under the same model can have different number of additional $CNOT$ gates and corresponding connections -- Fig. \ref{circuit_diagram} provides examples of different variants of the core classifier circuit. Each heterogeneous variant therefore has a different hyper-dimensional search space to optimize over and a different set of minima, resulting in a diverse set of core classifiers with different structures and parameters. The output of these variants can be combined by integrating \sol{}'s bitwise core classifiers with the weighted ensemble averaging, as expressed below:
\begin{equation}
\hat{y} = \sum_{b=0}^{n}2^{n-b}\Bigg[\dfrac{sgn\Big(\sum_{\epsilon}  \dfrac{a_\epsilon}{a}  q_{b\epsilon}\Big)+1}{2}\Bigg]
\end{equation}
Fig.~\ref{definitions} provides a visual representation of the diversity hierarchy of a model, a variant, and an instance. Different models are the most diverse due to them optimizing different objectives. However, for \sol{}'s ensemble, we need all core classifier models to have the same objective. Therefore, \sol{} employs different variants that are part of the same model (i.e., have the same objective) and provide better diversity than just having different instances.\vspace{2mm}


%\noindent\textbf{Multiple Instances of Core Classifiers.} \textit{\sol{}'s approach to remedy the aforementioned issue of scaling is to create an ensemble of core classifiers, each with the same objective, but with different initial conditions, leading to different parameters.} These instances enable an ensemble approach that works in improving accuracy by adding redundancies to blind spots in each classifier. Integrating \sol{}'s bitwise classification with the ensemble can be expressed as:
%\begin{equation}
%\hat{y} = \sum_{b=0}^{n}2^{n-b}\Bigg[\dfrac{sgn\Big(\sum_{\epsilon}  \dfrac{a_\epsilon}{a}  %q_{b\epsilon}\Big)+1}{2}\Bigg]
%\end{equation}

%XXX-- this whole paragraph is confusing and unclear; unsure why instances are introduced before variants but in the reverse order in the figure. Also, hetero architecture is a variant thing why is it being discussed here? 
%In the case of scaling to three instances and using unweighted majority rules as a decision procedure, the probability of a correct guess with average accuracy $A$ for each classifier if independent, would be $P(\text{Correct}) = A^2(3-2A)$.  This theory does not translate perfectly in practice as some samples of data simply have a higher level of difficulty than others. \textit{\sol{} uses heterogeneous network architecture so that each model has different local and global minima to achieve in gradient descent based training.} \sol{} provides a few variations of architecture to enable this heterogeneous ensemble based on variants of the same model.--XXX.\vspace{2mm} XXX-- lead up to variants is missing; missing connection---XXX.

%\noindent\textbf{Multiple Variants of Core Classifiers.} The intuition behind a diverse ensemble is that an outcome is greater than the sum of its parts if the parts are unique. Initializing model instances with different initial conditions enforces a degree of diversity. \sol{} goes one step further by constructing model variants with different architectures in order to establish more diversity and independence between them. These variants differ in that each variant under the same model can have different number of additional $CNOT$ gates and corresponding connections. The intuition being XXX- what does this mean \textit{even if all the models start at different positions in the hyper-dimensional space, the global minimum would be the same regardless and therefore, would be less valuable to combine the insights of identical classifiers.} Fig. \ref{circuit_diagram} provides examples of different variants of the core classifier circuits. --XXX \vspace{2mm} 

\noindent\textbf{OneVsAll Classifiers for Error Correcting.} While core classifiers do most of the heavy lifting with classification, the addition of support networks to provide checks and balances helps improve the overall accuracy of the classification. \textit{One vs all (OneVsAll) classifiers are used for each class in order to provide a parity bit when necessary. These act as error correcting procedures that activate under certain conditions.} A OneVsAll classifier is a binary classifier where one class is assigned to one class and every other class is grouped together in the other class. In the case of \sol{}, there is one OneVsAll classifier for each class in the class space. These classifiers only act when the core classifiers have low confidence, defined by a confidence threshold, $\gamma$. This is shown in Eq. \ref{gamma_eq} and is applied to each image separately.
\begin{equation}
\Big{|} \sum_{\epsilon}  \dfrac{a_\epsilon}{a}  O(x,\theta)\Big{|}  < \gamma
\label{gamma_eq}
\end{equation}
We find the value of $\gamma$ is optimal when it is met for 10\% of all guesses. For all images, if any have an absolute sum of weighted outputs that falls within $\gamma$, we identify the least confident bit $b$ in the output as:
\begin{equation}
b = \operatorname*{argmin}_{b} \Big{|}\sum_{\epsilon}  \dfrac{a_\epsilon}{a}  O(x,\theta)\Big{|}
\end{equation}
The next step is to evaluate the associated OneVsAll classifier for a final verdict on the bit in question. As there is a single bit in question, two OneVsAll Classifiers that are charged with the decision. For example, in the case of evaluating the most significant bit where the two least significant bits are certain (e.g., X01), the output is either a 1 or a 5, so the 1VsAll and 5VsAll classifiers must be evaluated. The bit is only set if and only if both OneVsAll Classifiers being evaluated agree on a decision, otherwise it defaults to its original state. This is shown for classifiers $C_1$ and $C_2$ below.
\[
  q_b = \left.
  \begin{cases}
     0, & \text{for } C_1 = -1, C_2 = 1 \\
     1, & \text{for } C_1 =  1, C_2 = -1 \\
     q_b, & \text{otherwise }
  \end{cases}
  \right\}
\]
Here, $-1$ indicates that the image is in the specific OneVsAll class, and $1$ indicates that it is not in the class.

\subsection{Stitching Together the Ensemble}

Overall, \sol{} requires five core classifiers + $n$ OneVsAll classifiers to build an ensemble for $n$ classes. For example, for its eight-class ensemble, \sol{} requires 13 classifiers: five core classifiers (each is a different variant) and eight OneVsAll classifiers. \textit{The number of models required by \sol{} therefore scales linearly with the number of classes, as opposed to quadratically with the state-of-the-art approach (Fig.~\ref{fig:onevone})}. \sol{}'s models construct a robust scalable ensemble with error correction built in. Next, we describe the implementation of our training and inference procedure.

%\sol{}'s network architecture can be segmented into three sections.  The first part of the network is the amplitude embedding, where the features are encoded onto the qubits. This is then followed by a repeating number of cascading layers that will be tuned. These layers are what are actually learning how to classify the data. Finally, measurement gates are used to measure the quantum state at the end of the inference or training procedure.  For core classifiers, \sol{} uses $log_{2}N$ measurement gates where $N$ is the number of classes.  OneVAll classifiers perform a binary classification and only require a single measurement gate.

%\subsection{Objective Function}
 
\subsection{Training and Inference Procedure}

%Due to the long wait times of reserving quantum machines, we opt to perform the entire training procedure on a quantum simulator. We reserve the use of quantum machines for running inference and performing the classifications, although it should be noted that the training procedure can be performed on quantum machines as well.

\sol{} begins by constructing the core model variants, each set to a learning rate of .05, optimized using the Adam optimizer~\cite{kingma2014adam}.  This is followed by randomly initializing all variants' weights separately between 0 and 1. For 100 epochs, these variants sample 50 random images and corresponding labels from the training set split. All vectorized images are passed into the network for evaluation. Within the context of the hybrid quantum-classical framework, gradients are computed classically after generating the outputs of the circuit. The new gate parameters are then optimized by shifting along the gradient to estimate the eigenvalues, then repeating until the optimization has terminated. \sol{} uses a form of a squared $L_2$ loss to perform gradient descent optimization. We find that squared loss works the best in training these small classification networks and outperforms $L_1$ loss or even techniques enforcing sparsity, such as the $L_0$ norm. The way \sol{} incorporates $L_2$ loss in binary classification for a single batch is as follows:
\begin{equation}
\text{Loss} = \sum_{i=0} ^{\text{batch}}(\text{label}[i] - \text{prediction}[i])^2\notag
\end{equation}
For more than two classes, the squared loss is summed over all output qubits $N$ used in the classification: 
\begin{equation}
\text{Loss} = {\sum_{i=0}^{\text{batch}}\sum_{j=0}^{N}}{(\text{label}[i][j] -\text{prediction}[i][j])^2}
\end{equation}
As an instance, in the eight-class case, this translates to only training the optimizer against the outputs of the first three qubits and ignoring the last two. As training these types of sensitive quantum networks does not provide a reliable advantage from one epoch to the next, we save the weights for the running best model.

To train the OneVsAll classifiers, we sample the labels to create an equal amount of data in both classes of the classifier. For example, to classify a ``7'' with 1000 images, the training set would consist of 1000 images of ``7'' and 1000 images composed of all other digits. These classifiers are also optimized using the Adam optimizer with $L_2$ loss.

In terms of inference, \sol{} runs the five trained core classifiers for each inference task and takes the weighted average of their output. If it determines that there exist bits with low confidence, \sol{} runs the respective OneVsAll classifiers for the bit with the lowest confidence. Once the final output is produced, \sol{} assesses all the classifier outputs and generates the final label for the inference task.
